RiSi: Spectro-temporal RAN-agnostic Modulation Identification for OFDMA Signals

RAN-agnostic communications can identify intrinsic features of the unknown signal without any prior knowledge, with which incompatible RANs in the same unlicensed band could achieve better coexistence performance than today's LBT-based coexistence. Blind modulation identification is its key building block, which blindly identifies the modulation type of an incompatible signal without any prior knowledge. Recent blind modulation identification schemes are built upon deep neural networks, which are limited to single-carrier signal recognition thus not pragmatic for identifying spectro-temporal OFDMA signals whose modulation varies with time and frequency. Therefore, this paper proposes RiSi, a semantic segmentation neural network designed to work on OFDMA's spectrograms, that employs flattened convolutions to better identify the grid-like pattern of OFDMA's resource blocks. We trained RiSi with a realistic OFDMA dataset including various channel impairments, and achieved the modulation identification accuracy of 86% on average over four modulation types of BPSK, QPSK, 16-QAM, 64-QAM. Then, we enhanced the generalization performance of RiSi by applying domain generalization methods while treating varying FFT size or varying CP length as different domains, showing that thus-generalized RiSi can perform reasonably well with unseen data.

==> dg.tex <==
Until now, we have only considered OFDM signals with an FFT size of 64 and a cyclic prefix (CP) length of 8.
%In practice, however, 
However, RAN-agnostic communication systems may be involved with numerous parameters (e.g., FFT size, CP length, etc.) that may vary according to protocol configurations and operation environments.
Therefore, we need to make RiSi to perform satisfactorily even with diverse signal parameter values that may not be seen in advance at the time of training. 
Unfortunately, this cannot be fulfilled by simply employing a larger dataset with more parametric variations, since a manageable-sized dataset cannot fully represent all possible combinations of parameter values.
Moreover, even slight modifications to system parameters can significantly alter the appearance of the resulting spectrogram, thus deteriorating RiSi's performance.

In this regard, this section investigates how to promote the ability of RiSi in extrapolating the signals unseen at the training stage.
Specifically, we address the issue of RiSi generalization as a `domain generalization (DG)' problem, by treating varying system parameters (i.e., OFDM FFT size and CP length) as different domains.
In doing so, we consider the same set of modulation classes while dealing with diversified spectrograms originating from the varying system parameters.

%Typically, a communication system is involved with numerous parameters (e.g., FFT size, CP length, etc.), but nevertheless we would like our proposed \textcolor{blue}{model} to perform well under various communication environments.
%%A typical communication system has numerous parameters and ideally we would like our network to perform well under any conditions.
%However, it is practically infeasible to fulfill the wish by simply employing a larger dataset with more diverse parametric variations, since a manageable-sized dataset cannot fully represent all possible combinations of parameter values.
%%However it is practically infeasible to create a finite dataset that includes signals representing an infinite number of possible parameter combinations for the network to learn.
%%Moreover, as it will be shown in VI-B, even slight modifications to system parameters can significantly alter the appearance of the resulting spectrogram, thus deteriorating the network performance.
%
%Therefore, it is necessary to study the ability of our network to extrapolate the signals unseen at the training stage.
%%To do so, we utilize the same modulation classes that need to be recognized across the spectrograms of varying system parameters.
%Accordingly, we can address the issue of \textcolor{blue}{generalization of RiSi for unseen communication system parameters,} as a Domain Generalization (DG) problem by treating system parameters such as OFDM FFT size as different image domains.


\subsection{Primer on Domain Generalization Techniques}

In the AI community,
%it has been known that machine learning \textcolor{blue}{models} suffer a significant performance \textcolor{blue}{degradation} when the test \textcolor{blue}{samples} lies outside of the training distribution \cite{temp1}. \textcolor{blue}{Specifically, 
the DG task pursues to train models on `train domains' for achieving better performance on `test domains' which have not been encountered during training.
Prior DG approaches mainly focus on computer vision applications where each domain indicates a distinctive image style such as photograph, sketch, etc. 
To give popular methods, Meta-Learning Domain Generalization (MLDG) leverages \textit{learn-to-learn} ability of meta-learning \cite{mldg}, Domain Adversarial training of Neural Networks (DANN) \cite{dann} 
%and Polarization of Embeddings (POEM) \cite{poem} 
pursues to discard domain-specific image features, and MixStyle tries to mix different domains to rehearse novel domains \cite{mixstyle}.
In \cite{lostDG}, however, the authors showed that the classical Empirical Risk Minimization (ERM) with proper optimizations can outperform most of the prior methods. 
Built upon the ERM baseline, Stochastic Weight Averaging Densely (SWAD) aims to search the network weights located at the flatter loss surface, which has been reported to enhance generalization \cite{swad}.

Among various DG approaches, we hereby focus on model- and task-agnostic methods such as ERM \cite{lostDG}, MLDG \cite{mldg}, SWAD \cite{swad}, which can be easily applied to our communication-specific task. 
Accordingly, we consider three ways of combining RiSi with a DG method as follows.
%We combine our RiSi with these DG methods to further evaluate the generalization capability to unseen communication parameters.
\begin{itemize}
\item \textbf{RiSi-ERM:} ERM is a general learning principle, which learns to minimize the total loss on train domains. Likewise, RiSi-ERM has been trained to minimize the loss on various communication parameters in train domains.
\item \textbf{RiSi-MLDG:} By following MLDG, for each training iteration, we randomly split the various communication parameters in train domains into `meta-train domain' and `meta-validation domain'. After training on a batch of meta-train domain samples, the network is then validated on meta-validation domains. We trained RiSi-MLDG with the meta-train and validation process.
%MLDG is based on Model-Agnostic Meta-Learning \cite{MAML}. 
%The final update of the model is computed by the weighted sum of the losses on meta-train and meta-validation. 
%Thus, the model is encouraged to learn the meta-train domains, while ensuring the improved generalization on meta-validation. 
\item \textbf{RiSi-SWAD:} SWAD is an ensemble-based DG method, which simply takes the average of a series of model weights obtained throughout conventional gradient-descent training. Its tolerance rate is for controlling the window of model weights to be averaged. We simply trained RiSi through the ensemble process of SWAD.
%which is shown to achieve flatter minima. 
%works as an important hyperparameter. 
%It was proved in \cite{swa} that such averaging would result in a model that achieves the flat minimum, thus making it more robust to changes caused by a domain shift.
%is an extension of SWA(Stochastic Weight Averaging) \cite{swa} to domain generalization. %It was shown to outperform previous models including ERM by a margin of 2\%. 
\end{itemize}

%We hereby choose to compare the performance of ERM, MLDG, and SWAD, since we believe they can best represent a wide variety of domain generalization methods. 

It is noteworthy that RiSi-ERM and RiSi-SWAD have an advantage against RiSi-MLDG thanks to their simplicity without defining meta-train/validation domains.
%On the contrary, \textcolor{blue}{RiSi-MLDG} may have problems due to the large number of potential domains that can be defined over the communication system and the way those domains may relate or interact with each other.

% Figure dg1: vertical axis - accuracies in %, horizontal axis - domain FFT size.


\subsection{RiSi's Domain Generalization Performance}

%Until now, we have only considered OFDM signals with an FFT size of 64 and a cyclic prefix (CP) length of 8.
%For practical RAN-agnostic communications, however, we need to make our network to work satisfactorily with various signal parameters which may not be known in advance. %, including OFDM's FFT size and cyclic prefix length.

An OFDMA signal could have completely different spectrograms if subcarrier spacing or the CP length is changed, which suggests that the FFT size and the CP length have a great impact on the domain-generalized performance.
Therefore, we hereby treat either `varying FFT sizes' or `varying CP lengths' as different domains.

%Here, we only consider 10k training dataset.


%---< COMBINED due to page limit of 7 >------------------------
\begin{figure}[!t]
\centering
  \subfigure[varying FFT size]{
    \includegraphics[width=0.488\columnwidth]{figures/fft_dg_CUT2.png}
%    \includegraphics[width=0.48\columnwidth]{figures/fft_dg_CUT2.png}
    \label{fft_dg}
    }
%  \hspace{-0.084in}    
  \hspace{-0.15in}    
  \subfigure[varying CP length]{
    \includegraphics[width=0.472\columnwidth]{figures/cp_dg_CUT2.png}
%    \includegraphics[width=0.464\columnwidth]{figures/cp_dg_CUT2.png}
    \label{cp_dg}
    }
\vspace{-0.15in}
\caption{Generalization performance of RiSi on varying FFT size and CP length. In (a), the vertical dashed lines imply the FFT sizes in the train domain. In (b), the lefthand side of the vertical dashed line construct the train domain.}
\label{fft_cp_dg}
%\vspace{-0.05in}
\end{figure}
%----------------------------------------------------------------------

%---< Moved to 'COMBINED' >--------------------------------------------
%\begin{figure}[!t]
%\centering
%\includegraphics[width=0.82\columnwidth]{figures/fft_dg_CUT.jpg} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes.
%\vspace{-0.1in}
%\caption{Generalization performance of RiSi-based methods on varying FFT size. The vertical dashed lines imply the FFT sizes in the train domain.}
%\label{fft_dg}
%\vspace{-0.05in}
%\end{figure}
%----------------------------------------------------------------------

\textbf{Varying FFT sizes:} We first assume a fixed CP length of 8 to focus on varying `FFT size' domains. 
The maximum FFT size used in the train domain is limited in the range from 8 to 64, while setting the test signals with larger FFT sizes up to 128 as the test domain which serves as out-of-domain cases.
We compare the performance of RiSi-ERM, RiSi-MLDG, and RiSi-SWAD when trained on the train domains with FFT sizes of 8, 12, 16, 24, 32, 48, and 64, while using an initial learning rate of 0.002 in all three models. 
For RiSi-ERM, the learning rate is exponentially decaying with a factor of 0.92. %and the model is trained until convergence; 
For RiSi-SWAD, the model is trained in the same way as RiSi-ERM for 10 epochs and then trained with a constant learning rate of 0.001 with the tolerance rate of 1.1.
For RiSi-MLDG, one meta-valiadation domain left out at each training iteration.
%, and use oracle validation (i.e., validating on the test set and choosing a model with the best performance).
%since \textcolor{blue}{RiSi-MLDG} does not define a stopping criterion.
%
As shown in Fig. \ref{fft_dg}, RiSi-SWAD is always performing better than RiSi-ERM, while RiSi-MLDG's performance is not promising except for the FFT sizes larger than 80.
%\textcolor{red}{applying domain generalization techniques like SWAD and MLDG leads to improvements in out-of-domain accuracies with FFT sizes larger than 80, while .

%----------------------------------------------------------------------
\if false
To justify the sampled source domains (i.e., `sparse') for training instead of using all available domains of $8,9,\ldots,64$ (i.e., `dense'), we trained \textcolor{blue}{RiSi-ERM} and \textcolor{blue}{RiSi-SWAD} for sparse and dense cases, respectively, as shown in Fig. \ref{dg2}.
% Fig dg2 - comparison of sparse domains with full domains
\textcolor{blue}{Although} dense training does achieve better accuracy than sparse training, the gap is smaller for RiSi-SWAD, and the sparse case performs better out-of-domain with FFT sizes larger than 64 in both SWAD and ERM cases.
Moreover, RiSi-SWAD trained on the sparse dataset is performing almost as good as the densely-trained RiSi-ERM in the train domain and has a superior performance in the test domain FFT sizes larger than 64.
We conjecture that the improved generalization with the sparse dataset is due to the model being overwhelmed with all the domains in the dense training set.
%
\begin{figure}
\centering
  \subfigure[RiSi-ERM: sparse vs. dense]{
    \includegraphics[width = 0.49\columnwidth]{./figures/erm_sparse_vs_dense.png}
    \label{10kacc}}
  \hspace{-0.25in}
  \subfigure[RiSi-SWAD: sparse vs. dense]{
    \includegraphics[width = 0.49\columnwidth]{./figures/swad_sparse_vs_dense.png}
    \label{10klosssdfbsdf}}
\caption{Training on dense and sparse datasets for RiSi-ERM and RiSi-SWAD}
\label{dg2}
\vspace{-0.1in}
\end{figure}
\fi
%----------------------------------------------------------------------

%---< Moved to 'COMBINED' >--------------------------------------------
%\begin{figure}[t]
%\centering
%\includegraphics[width=0.82\columnwidth]{figures/cp_dg_CUT.jpg} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes.
%\vspace{-0.1in}
%\caption{Generalization performance of RiSi-based methods on varying CP length. The lefthand side of the vertical dashed line construct the train domain.}
%\label{cp_dg}
%\vspace{-0.1in}
%\end{figure}
%----------------------------------------------------------------------


\textbf{Varying CP lengths:} Now, we fix the FFT size to 32 while varying the CP length.
%, which serves as different domains.
The train domain only contains the signals with a CP length ranging from 0 to 8, while the test domain has a full variety of CP lengths. 
%The results of this experiment are shown in Fig. \ref{cp_dg}.
As shown in Fig. \ref{cp_dg}, although the effect of the CP length domain shift is not as substantial as that of FFT size, there is still an improvement after applying the domain generalization methods.


\begin{table}
\centering
\begin{tabular}{ c|ccc }
\Xhline{3\arrayrulewidth}
  & Train domain & Test domain\\
 \hline\hline
 \textbf{RiSi-ERM} (varying FFT)   & 62.2\%    &45.9\%\\
 \textbf{RiSi-MLDG} (varying FFT) & 51.2\% & \textbf{47.7\%}\\
  \textbf{RiSi-SWAD} (varying FFT)&   \textbf{67.8\%}  & \textbf{47.7\%}\\
  \hline
 \textbf{RiSi-ERM} (varying CP)    & 70.9\% & 67.9\%\\
 \textbf{RiSi-MLDG} (varying CP)& 71.2\%  & 65.6\%\\
  \textbf{RiSi-SWAD} (varying CP)&   \textbf{74.4\%}  & \textbf{68.6\%}\\
\Xhline{3\arrayrulewidth}
% ERM& 60.9\%  & 44.7\%\\
% SWAD & 66.3\%& 46.0\%\\
% \hline
\end{tabular}
\vspace{0.1in}
\caption{Generalization for unseen FFT sizes and CP lengths}
\label{tb:dg_perf}
\vspace{-0.25in}
\end{table}

%Finally, we repeat our experiment with both FFT lengths and CP lengths varied.
Table~\ref{tb:dg_perf} summarizes the obtained mean accuracies for train and test domain performances, in the two training scenarios (i.e., varying FFT sizes and CP sizes). %, varying CP length and FFT size. 
We can confirm that DG methods, specifically RiSi-SWAD, allow us to improve test domain accuracy by approximately +1$\sim$2\%, while also improving train domain performance by +4$\sim$5\%, all compared to RiSi-ERM.
%Note, that there is no result for MLDG in the varying CP length and FFT size scenario. 
%This is because the necessary minibatch size in MLDG increases with the number of domains, and if both CP length and FFT size are varying, each combination of their possible values becomes a domain and the number of domains greatly increases. 
%Thus, the necessary minibatch size in MLDG increases making training complicated.
%We can also see that applying SWAD improves performance for both in-domain and out-of-domain cases.
RiSi-MLDG outperforms ERM in terms of test domain accuracy in the varying FFT scenario, but its overall performance is poor. 
In conclusion, RiSi-SWAD seems to be the best approach, consistently outperforming other cases. 
%We want to emphasize that our experiments for revealing the generalization of modulation recognition models to unseen communication scenario is the first attempt to investigate how the modulation recognition models are combined with the DG methods from AI research field, and what the resulting gain of the combinations is.


==> motivation.tex <==
Despite the high potential of blind modulation identification methods, how to utilize the recognized information for realizing RAN-agnostic coexistence is still an open issue. %in question.
In this regard, we introduce a simple but intuitive example of two incompatible RANs coexisting with each other, using which we will show how blind interference recognition enables RAN-agnostic rate adaptation of the two RANs and how much throughput gain it can achieve against the conventional SINR-based rate adaptation.
%SINR-based rate adaptation is today's de-facto standard for inter-RAN coexistence, where each RAN adapts its transmission parameters only according to the measured interference power.
%Therefore, when two incompatible RANs shares the same channel, their SINRs are significantly decreased and hence SINR-based rate adaptation has no choice but to downgrade its modulation to a less susceptible one to interference, e.g., from QPSK to BPSK.
In particular, we have devised multi-agent reinforcement learning (RL)-based RAN-agnostic rate adaptation where each RAN leverages RiSi to learn the intrinsic features of the other coexisting incompatible RAN, and exploits the obtained information to adjust its modulation and phase (e.g., adapting from the plain QPSK to a phase-tuned QPSK) so as to achieve better coexistence with the incompatible RAN.


\subsection{Intuitive Example for RAN-agnostic Rate Adaptation}
\label{subsec:toyexample}

\textbf{Setting:}
We consider two incompatible RANs, i.e., RAN1 and RAN2, each with a transmitter-receiver (TR) pair, as illustrated in Fig. \ref{fig:3-0}.
%We assume RAN1 is capable of RAN-agnostic rate adaptation while RAN2 follows SINR-based rate adaptation.
%\textcolor{red}{For RAN1, the distance between its transmitter and receiver (henceforth mentioned as `TR distance') is 10 meters, while the TR distance of RAN2 is 15 meters.
%In addition, the transmitter of RAN2 is 15 meters away from the receiver of RAN1, and the transmitter of RAN1 is 29 meters away from the receiver of RAN2.}
%This section deals with the toy example to determine the effect of interference signal identification.
%There exist two transmitter-receiver pairs for each of two incompatible RANs.
%For \textcolor{red}{the compatible RAN}, the distance between the transmitter and receiver nodes is 10 meters. 
%On the other hand, the receiver and transmitter nodes of \textcolor{red}{the incompatible RAN} are 15 meters apart from each other.
%The transmitter node of the incompatible RAN is 18 meters away from the receiver of the compatible RAN.
We assume each transceiver pair performs single-carrier transmission via a 20 MHz channel with the carrier frequency of 2.4 GHz, while the transmit power is initially set to 100 mW. 
In each channel, path-loss is modeled as $10 \gamma \log_{10}{(4\pi d / \lambda)}$ where $\gamma=2$ is the path-loss exponent, $d$ is the TR distance, and $\lambda$ is the wavelength. 
Also, each channel is assumed to experience Rician fading, where the ratio $K$ between the power of LoS (Line of Sight) path and that of other paths is set to 4 dB.
%\textcolor{blue}{When the transmitted signal $x$ is transmitted, the received signal through the channel vector $H$ is simply expressed as $y=Hx+n$, where $n\sim\mathcal{CN}(0,1)$ means AWGN.}
%\textcolor{blue}{Also, each channel is assumed to experience Rician fading, such as} %channel as a multi-path fading model.
%where the fading channel is given as}
%\begin{equation}
%\label{eq:ch_model_fading}
%H=\sqrt{\frac{K}{1+K}}\bar{H}+\sqrt{\frac{1}{1+K}}H_{f},
%\end{equation}
%\textcolor{blue}{where $\bar{H}$ is Line-Of-Sight (LOS) component and $H_{f}\sim\mathcal{CN}(0,1)$ is fading component with Rician $K$-factor $K=4$ dB.}
%\textcolor{red}{[HK: What is $H$ ?]}

\begin{figure}[!t]
\centering
%\includegraphics[width=1.0\columnwidth]{./figures/3-0.pdf}
\includegraphics[width=0.95\columnwidth]{./figures/3-0-1.png}
%\vspace{-0.2in}
\caption{Toy example scenario of RAN1-RAN2 coexistence}
\label{fig:3-0}
\vspace{-0.1in}
\end{figure}

\textbf{Conventional SINR-based rate adaptation:}
In the considered scenario, if a RAN would exist alone then it may choose QPSK as its modulation according to the measured SNR at its receiver.\footnote{We referred to the MCS(Modulation and Coding Scheme) table of IEEE 802.11ac, while considering assumed pass-loss and fading channel model.}
%with SINR-based rate adaptation, QPSK modulation is chosen by measuring the SNR at each RAN's receiver.
%If the two RANs operate with SINR-based rate adaptation, \textcolor{blue}{both RANs would use QPSK}, both based on the measured signal-to-noise ratio (SNR) at each RAN's receiver.
With two coexisting RANs sharing the same channel, however, the signal from RAN2's transmitter starts to interfere with RAN1's receiver, making the receiver's SINR significantly drop from $13.5$ dB to $2.33$ dB.
Similarly, RAN1's transmitter interferes with RAN2's receiver such that the receiver's SINR drops from $10.0$ dB to $2.82$ dB.
%In the case of SINR-based rate adaptation, RAN1 would fail to communicate, and RAN2 would have no choice but to downgrade its modulation to BPSK, risking reduced throughput. 
%\textcolor{blue}{Such a strategy to divide resources to avoid collision between incompatible RANs is a conventional approach that is widely used in resource allocation like time division multiplexing (TDM).}
With SINR-based rate adaptation, the severely degraded SINR at both sides implies they have to fall back to low-rate modulation like BPSK, if they try to transmit at the same time.
In the unlicensed band, LBT is adopted to avoid such inefficiency (i.e., both degraded to BPSK), where the two RANs alternatively access the channel thus forming a TDM(Time Division Multiplexing) like pattern.
%to rely on the conventional time division multiplexing (TDM) approach, where the given time resource is divided into two non-overlapping intervals, and each interval is assigned to each RAN.
With LBT, although each RAN can enjoy high performance with QPSK while it has an exclusive channel access, per-RAN throughput degrades much since a RAN's transmission opportunity is cut by half due to the time-shared access pattern between the two RANs.
As a result, the LBT-based conventional approach only achieves `2.0 bits per symbol' as the total sum-throughput of the two RANs.
%because each RAN selects QPSK, but the communication duration becomes half of the given interval.

%\textcolor{blue}{In an environment where bandwidth needs to be shared, over-low SINR forces the use of conventional resource allocation approache such as time division multiplexing (TDM).}
%\textcolor{red}{[HK: Do we want to discuss the following two separate strategies? 1) Keeping QPSK at both while time-sharing the channel, 2) Both transmitting simultaneously while degrading MCS.]}

%In case \textcolor{blue}{both RAN adopt} conventional rate adaptation, RAN2 would have no choice but downgrading its modulation to BPSK, risking reduced throughput.
%\textcolor{blue}{In case of RAN1, it wouldn't communicate with such low SINR.
%Therefore, in order for the two RANs to communicate, they must attempt communication by dividing time.}
%(2308 delete)\footnote{RAN2 may stay with BPSK even though its SINR drops from $4.5$ dB to $2.1$ dB due to the interference from RAN1's transmitter.}

%\textbf{Utilization of blind identification:}
\textbf{RAN-agnostic rate adaptation:}
We now describe how the blind modulation identification of incompatible RANs can enhance the coexistence performance. %with different RANs.
Specifically, we will show that 
with the help of blind modulation identification,
RAN1 with a phase-optimized BPSK and RAN2 with the plain QPSK can successfully coexist (i.e., they can transmit simultaneously), thus performing better than the LBT-based time sharing case.

As a baseline, if we simply force RAN1 with plain BPSK and RAN2 with plain QPSK to transmit at the same time, they fail to demodulate their received signals.
%We know that the two incompatible RANs catastrophically collapse.
As shown in Fig. \ref{fig:3-1}(a), the received QPSK symbol constellation of RAN2 is contaminated by the interfering BPSK signal from RAN1, where individually-colored four QPSK symbols (red, orange, blue, green) are shifted in two different directions due to the interfering BPSK resulting in an overlapped constellation, thus leading to failed demodulation.
In the mean time, RAN1 can achieve 0.98 bits per symbol, which is slightly degraded from the non-interfered BPSK case.

%The IQ-diagram in Fig. \ref{fig:3-1}(a) shows the received symbol constellations of \textcolor{blue}{the QPSK signal from RAN2} contaminated by \textcolor{blue}{the BPSK signal from RAN1}, where differently-colored four QPSK symbols are shifted in two directions due to interfering BPSK, resulting in an overlapped constellation thus leading to severely degraded demodulation performance.
%For anticipating the case of RAN-agnostic communications, let us assume that the receiver of RAN2 recognizes the modulation, phase, and power of the interference from RAN1.
Now, let us assume that each RAN's receiver can blindly recognize the interfering signal's modulation through RiSi.
Based on the learned knowledge, if RAN1 chooses to adapt its BPSK with a phase rotation by $\pi/4$, the received constellation of RAN2 becomes non-overlapped as shown in Fig.~\ref{fig:3-1}(b).
This permits successful demodulation of symbols via well-structured decision boundaries, i.e., when RAN2 recognizes RAN1's interference, it forms the decision boundaries as drawn and classifies each constellation cluster into the correct symbol.
As a result, RAN2 obtains 1.97 bits per symbol for the throughput, which is remarkably improved than the baseline, while RAN1 keeps achieving 0.98 bits per symbol.
Consequently, our method achieves `2.95 bits per symbol' in total, which is 1.475 times the conventional approach's 2.0 bits per symbol.

\begin{figure}[!t]
\centering
%\includegraphics[width=1.0\columnwidth]{./figures/3-1.pdf}
\includegraphics[width=0.99\columnwidth]{./figures/3-1-2-boundary.png}
\caption{The IQ-diagram of RAN2's received QPSK symbols when RAN1 is interfering with (a) plain BPSK, or (b) BPSK with optimized phase rotation}
\label{fig:3-1}
%\vspace{-0.05in}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=0.99\columnwidth]{./figures/3-1-3-boundary.png}
\caption{The IQ-diagram of RAN2's received QPSK symbols when RAN1 is interfering with (a) plain QPSK, or (b) QPSK with optimized phase rotation}
\label{fig:3-2}
\vspace{-0.1in}
\end{figure}

Likewise, we can also consider another baseline with both RANs using QPSK.
As a failure scenario, Fig.~\ref{fig:3-2}(a) shows the case where both RAN1 and RAN2 use plain QPSK.
On the other hand, we can find a successful coexistence scenario where RAN1 chooses QPSK with a phase rotation by $\pi/4$, which is shown in Fig.~\ref{fig:3-2}(b).
In this case, RAN1 and RAN2 achieve 1.91 and 1.93 bits per symbol, respectively, and hence the total throughput becomes `3.84 bits per symbol' in total, which is 1.92 times the conventional approach (and even better than 1.475 times!).
This suggests that depending on how we adapt modulations based on the learned information by RiSi, we may have various RAN-agnostic coexistence solutions.

Then, the remaining issue is how to build a practical algorithm that can adaptively find the optimal communication parameters of the two incompatible RANs to achieve the best coexistence, which is introduced in the sequel.

%With blind identification of the interference signal's modulation type, \textcolor{blue}{RAN2} can further enhance the coexistence performance by preserving its QPSK but with optimized phase rotation.
%\textcolor{blue}{We obtained a constellation as shown in Fig. \ref{fig:3-1}(b) by optimizing phase rotation.}
%To show the effect, suppose RAN1 recognizes RAN2's modulation type (i.e., BPSK) and runs RAN-agnostic rate adaptation to tune the plain \textcolor{blue}{BPSK} to a modified \textcolor{blue}{BPSK} with a phase rotation by \textcolor{blue}{$\pi/4$}, resulting in Fig. \ref{fig:3-1}(b).

%In other words, by utilizing the information of the identified interference signals, the RAN-agnostic method can find the phase-optimized modulation to get a non-overlapping symbol-wise clustering at the received signal constellation.
%\textcolor{blue}{In this example, our new approach obtained a throughput of 2.92, while TDM obtained a throughput of up to 2.0.}
%When the phase-optimized QPSK modulation is found by exhaustive searching, Fig. \ref{fig:3-2} presents the gains of the RAN-agnostic rate adaptation over the SINR-based approach. We plot the net throughput and Bit Error Rate (BER) curves, where the net throughput is the summation of the two RANs' throughput.


%%%%%%delete 231129
%\begin{figure}[!t]
%\centering
%\subfigure[]{
%\includegraphics[width=0.498\columnwidth]{./figures/3-3.png}
%\label{fig:3-2}
%}
%\hspace{-0.3in}
%\subfigure[]{
%\includegraphics[width=0.498\columnwidth]{./figures/3-4.png}
%\label{fig:3-3}
%}
%\caption{(a) Net-throughput graphs of two rate-adaptation methods (b) BER curves with or without phase optimization}
%\end{figure}

%%%%%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=0.85\columnwidth]{./figures/3-2.pdf}
%\includegraphics[width=0.70\columnwidth]{./figures/3-3.png}
%\vspace{-0.1in}
%\caption{Net-throughput graphs of two rate-adaptation methods}
%\label{fig:3-2}
%\vspace{-0.1in}
%\end{figure}
%\begin{figure}[!t]
%\centering
%\includegraphics[width=0.70\columnwidth]{./figures/3-4.png}
%\vspace{-0.1in}
%\caption{BER curves with or without phase optimization}
%\label{fig:3-3}
%\vspace{-0.1in}
%\end{figure}


% 231124 delete
%In general, the RAN-agnostic mechanism can evolve to optimize various communication parameters including modulation type, transmit power, phase rotation, etc.
%Nevertheless, this paper focuses on blind modulation identification, since it is the most fundamental building block of the RAN-agnostic communication technology while not fully investigated yet.
%Note that we reserve the problem of RAN-agnostic communication parameter optimization as our future work.


%In the cases without interference signal recognition, the decision line was classified as in-phase axis and quadrature axis in the same way as in conventional QPSK methods, and in cases with interference signal recognition, nearest classification based on the expected points in the IQ diagram is used. In case where interference signals are recognized identify 1.8 $dB$ gains in BER when SNR is 12 $dB$. 


%Each node is communicating with a power of 100 $mW$.
%Simulation uses the signals that are single-carrier settings, 2.4 $GHz$ frequency, and 20 $MHz$ bandwidth, and uses path-loss channel model (path loss exponent $\gamma=2$).

%If there is no interference signal, IQ-diagram at the receiver represents a typical form of QPSK modulation.
%However, the IQ-diagram when the presence of interference signal is shown in Fig.\ref{3-1}-(a).
%Since similar distances and similar powers, overlapping parts exist within IQ-diagram, which means that the error rate increases when two signals coexist.
%SINR(Signal-to-interference-plus-noise ratio) also dropped significantly from 8 $dB$ to 2.20 $dB$.
%When interference signal is not identified, communication can be attempted by changing modulation to BPSK or by increasing power, but former will reduce transfer efficiency and latter will drop SINR of the signal that treated as interference in this simulation.
%The conventional modulation selection method changes the modulation scheme from QPSK to BPSK when the SINR becomes lower.
%When only modulation methods are changed from QPSK to BPSK, BER reduces from $1.94\times10^{-1}$ to $2.35\times10^{-2}$, that means the effect of interference was reduced, but the modulation scheme changes resulted in about half efficiency.


%Identifying interference signals indicates that the location of each cluster can be estimated in IQ-diagram.
%This allows both communication to coexist while maintaining the QPSK scheme without changing the modulation method to BPSK.
%When the RAN nodes recognize the interference signal which use BPSK scheme with power of 100 $mW$ by interference identification, RAN nodes cannot be used QPSK scheme because of the premetioned reasons.
%Thus, modulation in a modified way is considered, in this example, a modulation method with a phase change by $-\frac{\pi}{6}$ is used.
%In the receiver, IQ-diagram as shown in Fig.\ref{3-1}-(b) can be obtained, and based on the location of each cluster that estimated by interference identification, nearest classification can be used to estimate which symbol each sample corresponds to.


%Fig.\ref{3-2} shows the BER graph for each of the aforementioned methods.
%The dotted line represents the BER when the QPSK modulation scheme is maintained without interference signal recognition, the solid line marked with circles is BER when the modulation scheme is changed to BPSK, and the solid line marked with squares is BER when the interference signal is recognized and the modified QPSK modulation scheme used.
%In cases without interference signal recognition, the decision line was classified as in-phase axis and quadrature axis in the same way as in conventional QPSK methods, and in cases with interference signal recognition, nearest classification based on the expected points in the IQ diagram is used.
%In case where interference signals are recognized identify 1.8 $dB$ gains in BER when SNR is 12 $dB$. 
%This indicates that the two RANs can coexist while maintaining transfer efficiency and maintaining power by not changing modulation methods.

%The toy example simulation above was carried out in a single carrier setting, but showed sufficient results as an example that motivated the need for interference signal recognition.
%By obtaining the information of the interference signal in advance, it is possible to select a modulation scheme to reduce errors during demodulation, which can be applied to RAN-agnostic communication to allow multiple RANs to coexist.


\subsection{Multi-agent RL-based RAN-agnostic Rate Adaptation}
\label{subsec:RLwithRiSi}

Built upon the toy example, we hereby provide an experiment to utilize multi-agent RL for RAN-agnostic rate adaptation
%, where an RL agent is deployed at each RAN-agnostic node (or possibly at the RAN controller like access point), and it 
that determines the communication parameters based on the recognized interference types.
%It is a non-trivial task due to the following reasons: i) RL agents should be fully decentralized both in training and testing. ii) The decision of one agent affects the reward of another agent.
%\textbf{Details of multi-agent RL:} 
Specifically, we assume that an RL agent is deployed at each RAN-agnostic transmitter, and RiSi provides the perfect blind modulation recognition.\footnote{Note that idealized RiSi is assumed since this is a preliminary study to show the potential of RAN-agnostic inter-RAN coexistence. Enhancement of RiSi's performance and RL combined with practical RiSi are our future work. Moreover, blind estimation of the phase offset in the received signal can be done after recognizing the modulation type, by applying various known techniques in the literature like \cite{SergienkoICASSP11}.} %of the interference signal is given by RiSi.
For each RL agent, we adopt the soft Actor-Critic model \cite{haarnoja2018soft} that takes the blind recognition result as inputs to select the optimal action among the following five choices: upgrade/downgrade modulation, increase/decrease phase, and keep modulation.
In a training episode, RAN1 and RAN2 sequentially tune their actions until they converge.

After sufficient training, the two RL agents, each governing its RAN's rate adaptation, indeed find the communication parameters to achieve the best inter-RAN coexistence.
When taking the average of 200 different test episodes, the average sum-throughput reached `3.60 bits per symbol', which is a little above the middle value between the performances of the two RAN-agnostic rate-adaptation cases in Figs.~\ref{fig:3-1} and \ref{fig:3-2} (i.e., 2.95 and 3.84).
%perfect transmissions of the two RANs with BPSK-QPSK and QPSK-QPSK coexistence cases. 
Furthermore, at each episode, we have confirmed that RL indeed converges to one of the two optimal coexistence solutions, which implies that the two possible solutions are almost equally selected by RL while the latter (i.e., RAN1 with phase-optimized QPSK and RAN2 with plain QPSK) is a bit more preferred.\footnote{Note that phase-optimized BPSK and phase-optimized QPSK might sometimes choose slightly different values than $\pi/4$ for the phase rotation, due to the randomness in the channel like fading.}
%
In addition, it is noteworthy to mention that the obtained sum-throughput of 3.60 bits/symbol is 1.80 times better than the conventional TDM-like approach. %, which shows 2 bits per symbol.

%As a result, the total throughput reaches \textcolor{red}{3.60 bits per symbol}, which is slightly below the perfect transmission of the two RANs \textcolor{red}{with QPSK modulation}.
%\textcolor{red}{The result is obtained by RL selecting BPSK-QPSK coexistence or QPSK-QPSK coexistence according to the situation for 200 test episodes.


%Specifically, RAN1 recognizes the interference from RAN2 and adapts its modulation by its RL agent. RAN2 then recognizes the newly-adapted interference from RAN1 and adapts its modulation. During a fixed coherence interval, the sequential process repeats until the two RANs decide to keep their modulation. In each episode, reward $R$ of each agent is the accumulation of the modified throughput of the corresponding RAN, i.e., $R=\text{(bits/symbol)}\times (1-BER)^{c}$, where $c=8$, which is empirically found.

%\textcolor{blue}{The two RL agents, where each governs the rate adaptation, indeed find the communication parameters that guarantee the coexistence of the two RANs.} 
%\textbf{Throughput gains of RL-based rate adaptation:} During 10,000 training episodes, the net throughput graph is shown in Fig. \ref{fig:3-5}.
%Surprisingly, the two RL agents, where each governs the rate adaptation, indeed find the communication parameters that guarantee the coexistence of the two RANs.

%%%%231129 delete
%\begin{figure}[!t]
%\centering
%\includegraphics[width=0.95\columnwidth]{./figures/3-5.png}
%\caption{Average net-sum throughput for test episodes}
%\label{fig:3-5}
%\vspace{-0.1in}
%\end{figure}

%We note that the main goal of our initial experiment is to provide intuitions of how RAN-agnostic communication can possibly be realized by utilizing the bling recognition technique, which emphasizes the importance of advanced interference identification.
In summary, our experiments provided an evidence that RAN-agnostic communications through blind modulation recognition can be realized by combining RiSi with RL, and can achieve optimal inter-RAN coexistence.
%We leave it as our future work to develop the overall system of RAN-agnostic communications, including blind modulation recognition, more sofisticated RL modules, and the protocol designs thereof.
%In this paper, we focus on developing an improved blind recognition method called RiSi, which potentially plays a key role in RAN-agnostic communications.


\subsection{Envisioning RAN-agnostic Communications Framework}

\begin{figure}[!t]
\centering
\includegraphics[width=0.99\columnwidth]{./figures/Framework.png}
\caption{Our vision of RAN-agnostic communications framework}
\label{fig:framework}
\vspace{-0.1in}
\end{figure}

Finally, we provide our vision on future RAN-agnostic communications for inter-RAN coexistence as follows.
As shown in Fig.~\ref{fig:framework}, each RAN-agnostic node would be equipped with RiSi and RaCE, where RaCE is the RL module that adapts transmission parameters according to what RiSi has identified as discussed earlier in this section.
We also expect RiSi can be further enhanced to become capable of identifying multiple mixed incompatible signals, which may be achieved by combining RiSi with blind source separation schemes in the literature \cite{LiuSensors21,PangJASP22,MaPhyCom22}.
Moreover, the RAN-agnostic nodes belonging to the same RAN could be coordinated to achieve better identification performance as they can provide various views of a given interfering signal.

Note that we leave it as our future work to develop signal-separating RiSi, RaCE, coordinated RiSi, and 
their protocols.
%the protocols thereof.





%======================================================

\if false

%Therefore, instead of Q-learning which is a value-based algorithm, 
%Each agent sequentially changes the modulation method, and each learns to increase throughput while ensuring a low BER.During training, the fading channel changes when the episode changes, and one episode is assumed to be within the coherent time. Within the episode, the two RANs may choose to change their modulation type or perform phase rotation sequentially. Whenever the model trains 100 episodes, 200 fixed various episodes are provided as test episodes to record the average of final net-sum throughput of the agents.

It improved to about 1.8 times better throughput than when communicating by dividing time in the conventional communication method.

In general, the RAN-agnostic mechanism can evolve to optimize various communication parameters including modulation type, transmit power, phase rotation, etc.
\textcolor{blue}{If the blind modulation identification focused in this paper is preceded, the problem of RAN-agnostic communication parameter optimizations can perform as the future works.}

\begin{figure}[!t]
\centering
\includegraphics[width=0.9\columnwidth]{./figures/3-5.png}
\caption{Average net-sum throughput for test episodes}
\label{fig:3-5}
\vspace{-0.1in}
\end{figure}


\subsection{Multi Agent Reinforcement Learning: Background}
\label{subsec:multiRL}
\textcolor{blue}{Reinforcement learning(RL) is learning paradigm to find a action direction for an agent to maximize the reward for action in a given state through trial and error.
RL is quite extensive and numerous algorithms have been presented.
Depending on the number of agents, it can be distinguished into single agent RL and multi-agent RL.
Most tasks in the world, such as autonomous driving and strategic games, are generally multi-agent environments.
In multi-agent RL, the action of other agents is also recognized as a change of the environment.
Due to this non stationarity, despite long research on RL, RL in a multi-agent environment still remains a challenge.}

\textcolor{blue}{Multi-agent RL is also closely related to game theory in that it explores situations in which individual choices affect the rewards of others.
Game theory classifies the environment in various ways.
Representatively, the environment can be classified into a cooperative game and a non-cooperative game.
The cooperative game is a game in which multi-agents cooperate with each other to increase a common reward, and the non-cooperative game is a game in which each agent does not communicate with each other and has its own reward.
If each agent's observations are different, it is naturally classified as an imperfect information game.
In the non-cooperative game, since each agent does not know the rewards of the other agents, game theory aims to find a Nash equilibrium in which each agent makes the best choice according to the counterpart's response, and eventually all agents do not change their choice \cite{nash1951non}. }

\textcolor{blue}{There are also various learning approaches for multi-agent RL.
\begin{itemize}
    \item Fully centralized
    \item Fully decentralized
    \item Centralized Training and Decentralized Execution (CTDE)
\end{itemize}
Fully centralized is a method of learning with one agent that oversees the whole, that is, a centralized controller, and fully decentralized is a learning method using a local policy for each agent.
CTDE is a method of learning using all observation information during training and using only the learned local policy during execution.
In most multi-agent RL studies, algorithms are constructed based on CTDE such as COMA\cite{foerster2018counterfactual}.
}
%%
%\textcolor{blue}{There are also various learning approaches for multi-agent RL.
%The first is the fully centralized method. It has the advantage of being a perfect information environment because it checks all states in a way that determines the state of %all agents and determines the action of each agent, but it has the disadvantage of increasing the joint action space exponentially.
%Conversely, the fully decentralized method is difficult to learn to cooperate or compete with each other agents in a way that each agent determines its action, and even if the Nash equilibrium is reached, there is also a possibility that this is a local maxima.
%Due to the shortcomings of the above two methods, most multi-agent reinforcement learning studies, such as COMA\cite{foerster2018counterfactual}, use Centralized Training and Decentralized Execution(CTDE) mechanism which use the observation information of all agents during training and use only the observation information of each agent in the execution process.
%Our experimental environment corresponds to fully decentralized method as an environment where observation information of other agents is difficult to use.}


\subsection{Reinforcement Learning for RAN-agnostic rate adaptation}
\label{subsec:multiRLexp}
\textcolor{blue}{In terms of game theory, our environment in Section~\ref{subsec:toyexample} can be said to be a non-cooperative game and should be learned in a fully decentralized, since each agent cannot communicate with each other in all training and execution processes.
In order to apply multi-agent RL in our setting, the simplest way is to apply the method of single agent RL as it is.
\cite{tan1993multi} performed independent Q-learning to each agent.
Our experimental environment is a fairly complex setting due to the randomness of the various fading channel.
Q-learning is a representative value-based algorithm, and the way the agent selects an action is deterministic.
On the other hand, the policy-based algorithm is stoichiometric in the method of selecting an action.
That is, the policy-based algorithm may have a more flexible policy than the value-based algorithm.
Therefore, instead of Q-learning which is a value-based algorithm, soft actor critic model\cite{haarnoja2018soft} was applied to each agent independently.
Each agent sequentially changes the modulation method, and each learns to increase throughput while ensuring a low BER.
During training, the fading channel changes when the episode changes, and one episode is assumed to be within the coherent time.
Within the episode, the two RANs may choose to change their modulation type or perform phase rotation sequentially.
Whenever the model trains 100 episodes, 200 fixed various episodes are provided as test episodes to record the average of final net-sum throughput of the agents.
After training 10,000 episodes, the graph obtained is shown in Fig. \ref{fig:3-5}.
It improved to about 1.8 times better throughput than when communicating by dividing time in the conventional communication method.
}

In general, the RAN-agnostic mechanism can evolve to optimize various communication parameters including modulation type, transmit power, phase rotation, etc.
\textcolor{blue}{If the blind modulation identification focused in this paper is preceded, the problem of RAN-agnostic communication parameter optimizations can perform as the future works.}

\fi
